Landscape Analysis for Surrogate Models in the Evolutionary Black-Box Context

Surrogate modeling has become a valuable technique for black-box optimization tasks with expensive evaluation of the objective function. In this paper, we investigate the relationship between the predictive accuracy of surrogate models and features of the black-box function landscape. We also study properties of features for landscape analysis in the context of different transformations and ways of selecting the input data. We perform the landscape analysis of a large set of data generated using runs of a surrogate-assisted version of the Covariance Matrix Adaptation Evolution Strategy on the noiseless part of the Comparing Continuous Optimisers benchmark function testbed.

==> Makefile <==
FNAME = pitra2022ec

OUT = $(FNAME).pdf
SRC = $(FNAME).tex
BIB = $(FNAME).bib
BIB_AUX = $(FNAME).aux
BIB_BBL = $(FNAME).bbl
DVI = $(FNAME).dvi
TMP = $(BIB_AUX) $(BIB_BBL) $(FNAME).log $(FNAME).blg $(FNAME).out

RM	 = /bin/rm -f

single: $(OUT)

pdf: $(OUT)

images/%_pproc.gv: images/%_ecml.gv
	dot2tex -f tikz -t raw -s  --preproc --tikzedgelabels --figonly $< > $@

tex/%.tex: images/%_pproc.gv
	dot2tex -f tikz -t raw -s --tikzedgelabels --figonly $< > $@

tex/tree_full_postproc.tex: tex/tree_full.tex
	sed 's/-- node/-- node\[right, outer sep=2bp\]/' $< > $@

tex/tree_nearest_postproc.tex: tex/tree_nearest.tex
	sed 's/-- node/-- node\[right, outer sep=2bp\]/' $< > $@

$(OUT): $(SRC) $(BIB_BBL) tex/tree_full_postproc.tex tex/tree_nearest_postproc.tex tex/*.tex images/*.pdf
	pdflatex $(SRC)
	pdflatex $(SRC)

all: clean $(OUT) postscript

$(BIB_BBL): $(BIB)
	pdflatex $(SRC)
	bibtex $(BIB_AUX)
	pdflatex $(SRC)

display: $(OUT)
	open $(OUT) # Platform dependent

postscript: $(SRC) $(BIB_BBL)
	latex $(SRC)
	dvips $(DVI)

clean:
	$(RM) $(OUT) $(TMP)
clean_tmp:
	$(RM) $(TMP)


==> tex/clusterTable.tex <==
\begin{tabular}{rlrlrl}

\toprule

\multicolumn{2}{c}{TSS full}                                                                                                & \multicolumn{2}{c}{TSS nearest}                                                                                                 & \multicolumn{2}{c}{TSS knn}                                                                                                 \\

\midrule

          \multirow{2}{*}{1} & \cellcolor[gray]{0.85} $\tableFeat{lda\_qda\_10}{\archivepred}{\transnone}{\text{\ftLevel}}$ &              \multirow{1}{*}{1} &                            \cellcolor[gray]{0.85} $\tableFeat{step\_size}{}{}{\text{\ftCMA}}$ &         \multirow{18}{*}{1} &                                                   $\tableFeat{step\_size}{}{}{\text{\ftCMA}}$ \\
\cmidrule(lr){3-4}
                             &                         $\tableFeat{lda\_qda\_10}{\archivepred}{\transcma}{\text{\ftLevel}}$ &              \multirow{4}{*}{2} &  \cellcolor[gray]{0.85} $\tableFeat{lda\_qda\_10}{\archivepred}{\transnone}{\text{\ftLevel}}$ &                             &                                   $\tableFeat{cma\_lik}{\archive}{\transnone}{\text{\ftCMA}}$ \\
\cmidrule(lr){1-2}
          \multirow{1}{*}{2} &                           \cellcolor[gray]{0.85} $\tableFeat{step\_size}{}{}{\text{\ftCMA}}$ &                                 &                          $\tableFeat{lda\_qda\_10}{\archivepred}{\transcma}{\text{\ftLevel}}$ &                             &                             $\tableFeat{diff\_mean\_05}{\archive}{\transcma}{\text{\ftDisp}}$ \\
\cmidrule(lr){1-2}
          \multirow{6}{*}{3} &                                  $\tableFeat{cma\_lik}{\archive}{\transnone}{\text{\ftCMA}}$ &                                 &                        $\tableFeat{lda\_qda\_10}{\trainpredset}{\transnone}{\text{\ftLevel}}$ &                             &                           $\tableFeat{diff\_median\_05}{\archive}{\transcma}{\text{\ftDisp}}$ \\

                             &                            $\tableFeat{diff\_mean\_10}{\archive}{\transcma}{\text{\ftDisp}}$ &                                 &                         $\tableFeat{lda\_qda\_10}{\trainpredset}{\transcma}{\text{\ftLevel}}$ &                             &      \cellcolor[gray]{0.85} $\tableFeat{diff\_mean\_10}{\archive}{\transcma}{\text{\ftDisp}}$ \\
\cmidrule(lr){3-4}
                             &                            $\tableFeat{diff\_mean\_25}{\archive}{\transcma}{\text{\ftDisp}}$ &              \multirow{8}{*}{3} &                             $\tableFeat{diff\_mean\_05}{\archive}{\transcma}{\text{\ftDisp}}$ &                             &                           $\tableFeat{diff\_median\_10}{\archive}{\transcma}{\text{\ftDisp}}$ \\

                             &                              $\tableFeat{cma\_lik}{\archivepred}{\transnone}{\text{\ftCMA}}$ &                                 &                           $\tableFeat{diff\_median\_05}{\archive}{\transcma}{\text{\ftDisp}}$ &                             &                             $\tableFeat{diff\_mean\_25}{\archive}{\transcma}{\text{\ftDisp}}$ \\

                             &                        $\tableFeat{diff\_mean\_10}{\archivepred}{\transcma}{\text{\ftDisp}}$ &                                 &  \cellcolor[gray]{0.85} $\tableFeat{diff\_mean\_05}{\archivepred}{\transcma}{\text{\ftDisp}}$ &                             &                           $\tableFeat{diff\_median\_25}{\archive}{\transcma}{\text{\ftDisp}}$ \\

                             & \cellcolor[gray]{0.85} $\tableFeat{diff\_mean\_25}{\archivepred}{\transcma}{\text{\ftDisp}}$ &                                 &                       $\tableFeat{diff\_median\_05}{\archivepred}{\transcma}{\text{\ftDisp}}$ &                             &                               $\tableFeat{cma\_lik}{\archivepred}{\transnone}{\text{\ftCMA}}$ \\
\cmidrule(lr){1-2}
          \multirow{4}{*}{4} &                            $\tableFeat{diff\_mean\_05}{\archive}{\transcma}{\text{\ftDisp}}$ &                                 &                            $\tableFeat{diff\_mean\_05}{\trainset}{\transcma}{\text{\ftDisp}}$ &                             &                         $\tableFeat{diff\_mean\_05}{\archivepred}{\transcma}{\text{\ftDisp}}$ \\

                             &                          $\tableFeat{diff\_median\_05}{\archive}{\transcma}{\text{\ftDisp}}$ &                                 &                          $\tableFeat{diff\_median\_05}{\trainset}{\transcma}{\text{\ftDisp}}$ &                             &                       $\tableFeat{diff\_median\_05}{\archivepred}{\transcma}{\text{\ftDisp}}$ \\

                             & \cellcolor[gray]{0.85} $\tableFeat{diff\_mean\_05}{\archivepred}{\transcma}{\text{\ftDisp}}$ &                                 &                        $\tableFeat{diff\_mean\_05}{\trainpredset}{\transcma}{\text{\ftDisp}}$ &                             &                         $\tableFeat{diff\_mean\_10}{\archivepred}{\transcma}{\text{\ftDisp}}$ \\

                             &                      $\tableFeat{diff\_median\_05}{\archivepred}{\transcma}{\text{\ftDisp}}$ &                                 &                      $\tableFeat{diff\_median\_05}{\trainpredset}{\transcma}{\text{\ftDisp}}$ &                             &                       $\tableFeat{diff\_median\_10}{\archivepred}{\transcma}{\text{\ftDisp}}$ \\
\cmidrule(lr){1-2}\cmidrule(lr){3-4}
          \multirow{4}{*}{5} &   \cellcolor[gray]{0.85} $\tableFeat{diff\_median\_10}{\archive}{\transcma}{\text{\ftDisp}}$ &             \multirow{12}{*}{4} &                                   $\tableFeat{cma\_lik}{\archive}{\transnone}{\text{\ftCMA}}$ &                             &                         $\tableFeat{diff\_mean\_25}{\archivepred}{\transcma}{\text{\ftDisp}}$ \\

                             &                          $\tableFeat{diff\_median\_25}{\archive}{\transcma}{\text{\ftDisp}}$ &                                 &                             $\tableFeat{diff\_mean\_10}{\archive}{\transcma}{\text{\ftDisp}}$ &                             &                       $\tableFeat{diff\_median\_25}{\archivepred}{\transcma}{\text{\ftDisp}}$ \\

                             &                      $\tableFeat{diff\_median\_10}{\archivepred}{\transcma}{\text{\ftDisp}}$ &                                 &                             $\tableFeat{diff\_mean\_25}{\archive}{\transcma}{\text{\ftDisp}}$ &                             &                     $\tableFeat{lin\_simple\_coef\_max}{\trainset}{\transnone}{\text{\ftMM}}$ \\

                             &                      $\tableFeat{diff\_median\_25}{\archivepred}{\transcma}{\text{\ftDisp}}$ &                                 &                               $\tableFeat{cma\_lik}{\archivepred}{\transnone}{\text{\ftCMA}}$ &                             &                            $\tableFeat{cma\_mean\_dist}{\trainset}{\transcma}{\text{\ftCMA}}$ \\
\cmidrule(lr){1-2}
          \multirow{4}{*}{6} &                            $\tableFeat{diff\_mean\_02}{\archive}{\transcma}{\text{\ftDisp}}$ &                                 &                         $\tableFeat{diff\_mean\_10}{\archivepred}{\transcma}{\text{\ftDisp}}$ &                             &                        $\tableFeat{cma\_mean\_dist}{\trainpredset}{\transcma}{\text{\ftCMA}}$ \\
\cmidrule(lr){5-6}
                             &   \cellcolor[gray]{0.85} $\tableFeat{diff\_median\_02}{\archive}{\transcma}{\text{\ftDisp}}$ &                                 &  \cellcolor[gray]{0.85} $\tableFeat{diff\_mean\_25}{\archivepred}{\transcma}{\text{\ftDisp}}$ &          \multirow{4}{*}{2} &                                    $\tableFeat{cma\_lik}{\archive}{\transcma}{\text{\ftCMA}}$ \\

                             &                        $\tableFeat{diff\_mean\_02}{\archivepred}{\transcma}{\text{\ftDisp}}$ &                                 &                                  $\tableFeat{cma\_lik}{\trainset}{\transnone}{\text{\ftCMA}}$ &                             &         \cellcolor[gray]{0.85} $\tableFeat{cma\_lik}{\archivepred}{\transcma}{\text{\ftCMA}}$ \\

                             &                      $\tableFeat{diff\_median\_02}{\archivepred}{\transcma}{\text{\ftDisp}}$ &                                 &                            $\tableFeat{diff\_mean\_10}{\trainset}{\transcma}{\text{\ftDisp}}$ &                             &                                   $\tableFeat{cma\_lik}{\trainset}{\transcma}{\text{\ftCMA}}$ \\
\cmidrule(lr){1-2}
          \multirow{1}{*}{7} &                              \cellcolor[gray]{0.85} $\tableFeat{restart}{}{}{\text{\ftCMA}}$ &                                 &                            $\tableFeat{diff\_mean\_25}{\trainset}{\transcma}{\text{\ftDisp}}$ &                             &                               $\tableFeat{cma\_lik}{\trainpredset}{\transcma}{\text{\ftCMA}}$ \\
\cmidrule(lr){1-2}\cmidrule(lr){5-6}
          \multirow{2}{*}{8} &                                   $\tableFeat{cma\_lik}{\archive}{\transcma}{\text{\ftCMA}}$ &                                 &                              $\tableFeat{cma\_lik}{\trainpredset}{\transnone}{\text{\ftCMA}}$ &          \multirow{2}{*}{3} &                                  $\tableFeat{cma\_lik}{\trainset}{\transnone}{\text{\ftCMA}}$ \\

                             &        \cellcolor[gray]{0.85} $\tableFeat{cma\_lik}{\archivepred}{\transcma}{\text{\ftCMA}}$ &                                 &                        $\tableFeat{diff\_mean\_10}{\trainpredset}{\transcma}{\text{\ftDisp}}$ &                             &       \cellcolor[gray]{0.85} $\tableFeat{cma\_lik}{\trainpredset}{\transnone}{\text{\ftCMA}}$ \\
\cmidrule(lr){1-2}\cmidrule(lr){5-6}
          \multirow{1}{*}{9} &                     \cellcolor[gray]{0.85} $\tableFeat{evopath\_s\_norm}{}{}{\text{\ftCMA}}$ &                                 &                        $\tableFeat{diff\_mean\_25}{\trainpredset}{\transcma}{\text{\ftDisp}}$ &          \multirow{2}{*}{4} &  \cellcolor[gray]{0.85} $\tableFeat{lda\_qda\_10}{\archivepred}{\transnone}{\text{\ftLevel}}$ \\
\cmidrule(lr){1-2}\cmidrule(lr){3-4}
         \multirow{1}{*}{10} &                     \cellcolor[gray]{0.85} $\tableFeat{evopath\_c\_norm}{}{}{\text{\ftCMA}}$ &              \multirow{8}{*}{5} &    \cellcolor[gray]{0.85} $\tableFeat{diff\_median\_10}{\archive}{\transcma}{\text{\ftDisp}}$ &                             &                          $\tableFeat{lda\_qda\_10}{\archivepred}{\transcma}{\text{\ftLevel}}$ \\
\cmidrule(lr){1-2}\cmidrule(lr){5-6}
         \multirow{2}{*}{11} & \cellcolor[gray]{0.85} $\tableFeat{lda\_qda\_25}{\archivepred}{\transnone}{\text{\ftLevel}}$ &                                 &                           $\tableFeat{diff\_median\_25}{\archive}{\transcma}{\text{\ftDisp}}$ &          \multirow{4}{*}{5} &     \cellcolor[gray]{0.85} $\tableFeat{diff\_mean\_05}{\trainset}{\transcma}{\text{\ftDisp}}$ \\

                             &                         $\tableFeat{lda\_qda\_25}{\archivepred}{\transcma}{\text{\ftLevel}}$ &                                 &                       $\tableFeat{diff\_median\_10}{\archivepred}{\transcma}{\text{\ftDisp}}$ &                             &                          $\tableFeat{diff\_median\_05}{\trainset}{\transcma}{\text{\ftDisp}}$ \\
\cmidrule(lr){1-2}
         \multirow{1}{*}{12} &                                               \cellcolor[gray]{0.85} $\tableFeat{dim}{}{}{}$ &                                 &                       $\tableFeat{diff\_median\_25}{\archivepred}{\transcma}{\text{\ftDisp}}$ &                             &                        $\tableFeat{diff\_mean\_05}{\trainpredset}{\transcma}{\text{\ftDisp}}$ \\
\cmidrule(lr){1-2}
         \multirow{3}{*}{13} &                                       \cellcolor[gray]{0.85} $\tableFeat{obs}{\archive}{}{}$ &                                 &                          $\tableFeat{diff\_median\_10}{\trainset}{\transcma}{\text{\ftDisp}}$ &                             &                      $\tableFeat{diff\_median\_05}{\trainpredset}{\transcma}{\text{\ftDisp}}$ \\
\cmidrule(lr){5-6}
                             &                                                  $\tableFeat{generation}{}{}{\text{\ftCMA}}$ &                                 &                          $\tableFeat{diff\_median\_25}{\trainset}{\transcma}{\text{\ftDisp}}$ &          \multirow{1}{*}{6} &                      \cellcolor[gray]{0.85} $\tableFeat{evopath\_s\_norm}{}{}{\text{\ftCMA}}$ \\
\cmidrule(lr){5-6}
                             &                                                          $\tableFeat{obs}{\archivepred}{}{}$ &                                 &                      $\tableFeat{diff\_median\_10}{\trainpredset}{\transcma}{\text{\ftDisp}}$ &          \multirow{2}{*}{7} &  \cellcolor[gray]{0.85} $\tableFeat{lda\_qda\_25}{\archivepred}{\transnone}{\text{\ftLevel}}$ \\
\cmidrule(lr){1-2}
         \multirow{1}{*}{14} &   \cellcolor[gray]{0.85} $\tableFeat{quad\_simple\_cond}{\archive}{\transcma}{\text{\ftMM}}$ &                                 &                      $\tableFeat{diff\_median\_25}{\trainpredset}{\transcma}{\text{\ftDisp}}$ &                             &                          $\tableFeat{lda\_qda\_25}{\archivepred}{\transcma}{\text{\ftLevel}}$ \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
                             &                                                                                              &              \multirow{1}{*}{6} &                      \cellcolor[gray]{0.85} $\tableFeat{evopath\_c\_norm}{}{}{\text{\ftCMA}}$ &          \multirow{3}{*}{8} &                     $\tableFeat{lin\_simple\_coef\_min}{\trainset}{\transnone}{\text{\ftMM}}$ \\
\cmidrule(lr){3-4}
                             &                                                                                              &              \multirow{5}{*}{7} &                                                               $\tableFeat{obs}{\archive}{}{}$ &                             &          \cellcolor[gray]{0.85} $\tableFeat{eps\_max}{\trainset}{\transnone}{\text{\ftInfo}}$ \\

                             &                                                                                              &                                 &                                                   $\tableFeat{generation}{}{}{\text{\ftCMA}}$ &                             &                             $\tableFeat{eps\_max}{\trainpredset}{\transnone}{\text{\ftInfo}}$ \\
\cmidrule(lr){5-6}
                             &                                                                                              &                                 &                                                           $\tableFeat{obs}{\archivepred}{}{}$ &          \multirow{1}{*}{9} &  \cellcolor[gray]{0.85} $\tableFeat{quad\_simple\_cond}{\trainset}{\transnone}{\text{\ftMM}}$ \\
\cmidrule(lr){5-6}
                             &                                                                                              &                                 &                                       \cellcolor[gray]{0.85} $\tableFeat{obs}{\trainset}{}{}$ &         \multirow{1}{*}{10} &                               \cellcolor[gray]{0.85} $\tableFeat{restart}{}{}{\text{\ftCMA}}$ \\
\cmidrule(lr){5-6}
                             &                                                                                              &                                 &                                                          $\tableFeat{obs}{\trainpredset}{}{}$ &         \multirow{8}{*}{11} &                            $\tableFeat{diff\_mean\_10}{\trainset}{\transcma}{\text{\ftDisp}}$ \\
\cmidrule(lr){3-4}
                             &                                                                                              &              \multirow{4}{*}{8} &                                    $\tableFeat{cma\_lik}{\archive}{\transcma}{\text{\ftCMA}}$ &                             &                          $\tableFeat{diff\_median\_10}{\trainset}{\transcma}{\text{\ftDisp}}$ \\

                             &                                                                                              &                                 &         \cellcolor[gray]{0.85} $\tableFeat{cma\_lik}{\archivepred}{\transcma}{\text{\ftCMA}}$ &                             &                            $\tableFeat{diff\_mean\_25}{\trainset}{\transcma}{\text{\ftDisp}}$ \\

                             &                                                                                              &                                 &                                   $\tableFeat{cma\_lik}{\trainset}{\transcma}{\text{\ftCMA}}$ &                             &                          $\tableFeat{diff\_median\_25}{\trainset}{\transcma}{\text{\ftDisp}}$ \\

                             &                                                                                              &                                 &                               $\tableFeat{cma\_lik}{\trainpredset}{\transcma}{\text{\ftCMA}}$ &                             & \cellcolor[gray]{0.85} $\tableFeat{diff\_mean\_10}{\trainpredset}{\transcma}{\text{\ftDisp}}$ \\
\cmidrule(lr){3-4}
                             &                                                                                              &              \multirow{1}{*}{9} &                      \cellcolor[gray]{0.85} $\tableFeat{evopath\_s\_norm}{}{}{\text{\ftCMA}}$ &                             &                      $\tableFeat{diff\_median\_10}{\trainpredset}{\transcma}{\text{\ftDisp}}$ \\
\cmidrule(lr){3-4}
                             &                                                                                              &             \multirow{1}{*}{10} &                                                \cellcolor[gray]{0.85} $\tableFeat{dim}{}{}{}$ &                             &                        $\tableFeat{diff\_mean\_25}{\trainpredset}{\transcma}{\text{\ftDisp}}$ \\
\cmidrule(lr){3-4}
                             &                                                                                              &             \multirow{4}{*}{11} &                         $\tableFeat{lda\_qda\_25}{\archivepred}{\transnone}{\text{\ftLevel}}$ &                             &                      $\tableFeat{diff\_median\_25}{\trainpredset}{\transcma}{\text{\ftDisp}}$ \\
\cmidrule(lr){5-6}
                             &                                                                                              &                                 &                          $\tableFeat{lda\_qda\_25}{\archivepred}{\transcma}{\text{\ftLevel}}$ &         \multirow{6}{*}{12} &                                                               $\tableFeat{obs}{\archive}{}{}$ \\

                             &                                                                                              &                                 & \cellcolor[gray]{0.85} $\tableFeat{lda\_qda\_25}{\trainpredset}{\transnone}{\text{\ftLevel}}$ &                             &                                                   $\tableFeat{generation}{}{}{\text{\ftCMA}}$ \\

                             &                                                                                              &                                 &                         $\tableFeat{lda\_qda\_25}{\trainpredset}{\transcma}{\text{\ftLevel}}$ &                             &                           $\tableFeat{quad\_simple\_cond}{\archive}{\transcma}{\text{\ftMM}}$ \\
\cmidrule(lr){3-4}
                             &                                                                                              &             \multirow{1}{*}{12} &                               \cellcolor[gray]{0.85} $\tableFeat{restart}{}{}{\text{\ftCMA}}$ &                             &                                    \cellcolor[gray]{0.85} $\tableFeat{obs}{\archivepred}{}{}$ \\
\cmidrule(lr){3-4}
                             &                                                                                              &             \multirow{8}{*}{13} &                             $\tableFeat{diff\_mean\_02}{\archive}{\transcma}{\text{\ftDisp}}$ &                             &                                                              $\tableFeat{obs}{\trainset}{}{}$ \\

                             &                                                                                              &                                 &                           $\tableFeat{diff\_median\_02}{\archive}{\transcma}{\text{\ftDisp}}$ &                             &                                                          $\tableFeat{obs}{\trainpredset}{}{}$ \\
\cmidrule(lr){5-6}
                             &                                                                                              &                                 &                         $\tableFeat{diff\_mean\_02}{\archivepred}{\transcma}{\text{\ftDisp}}$ &         \multirow{3}{*}{13} &                                                \cellcolor[gray]{0.85} $\tableFeat{dim}{}{}{}$ \\

                             &                                                                                              &                                 &                       $\tableFeat{diff\_median\_02}{\archivepred}{\transcma}{\text{\ftDisp}}$ &                             &                                             $\tableFeat{evopath\_c\_norm}{}{}{\text{\ftCMA}}$ \\

                             &                                                                                              &                                 &                            $\tableFeat{diff\_mean\_02}{\trainset}{\transcma}{\text{\ftDisp}}$ &                             &                       $\tableFeat{cma\_mean\_dist}{\trainpredset}{\transnone}{\text{\ftCMA}}$ \\
\cmidrule(lr){5-6}
                             &                                                                                              &                                 &   \cellcolor[gray]{0.85} $\tableFeat{diff\_median\_02}{\trainset}{\transcma}{\text{\ftDisp}}$ &         \multirow{4}{*}{14} &                             $\tableFeat{diff\_mean\_02}{\archive}{\transcma}{\text{\ftDisp}}$ \\

                             &                                                                                              &                                 &                        $\tableFeat{diff\_mean\_02}{\trainpredset}{\transcma}{\text{\ftDisp}}$ &                             &    \cellcolor[gray]{0.85} $\tableFeat{diff\_median\_02}{\archive}{\transcma}{\text{\ftDisp}}$ \\

                             &                                                                                              &                                 &                      $\tableFeat{diff\_median\_02}{\trainpredset}{\transcma}{\text{\ftDisp}}$ &                             &                         $\tableFeat{diff\_mean\_02}{\archivepred}{\transcma}{\text{\ftDisp}}$ \\
\cmidrule(lr){3-4}
                             &                                                                                              &             \multirow{2}{*}{14} &                           $\tableFeat{quad\_simple\_cond}{\archive}{\transcma}{\text{\ftMM}}$ &                             &                       $\tableFeat{diff\_median\_02}{\archivepred}{\transcma}{\text{\ftDisp}}$ \\

                             &                                                                                              &                                 &   \cellcolor[gray]{0.85} $\tableFeat{quad\_simple\_cond}{\trainset}{\transcma}{\text{\ftMM}}$ &                             &                                                                                               \\

\bottomrule

\end{tabular}


